CF-GKAT: Efficient Validation of Control-Flow Transformations

Guarded Kleene Algebra with Tests (GKAT) provides a sound and complete framework to reason about trace equivalence between simple imperative programs. However, there are still several notable limitations. First, GKAT is completely agnostic with respect to the meaning of primitives, to keep equivalence decidable. Second, GKAT excludes non-local control flow such as goto, break, and return. To overcome these limitations, we introduce Control-Flow GKAT (CF-GKAT), a system that allows reasoning about programs that include non-local control flow as well as hardcoded values. CF-GKAT is able to soundly and completely verify trace equivalence of a larger class of programs, while preserving the nearly-linear efficiency of GKAT. This makes CF-GKAT suitable for the verification of control-flow manipulating procedures, such as decompilation and goto-elimination. To demonstrate CF-GKAT's abilities, we validated the output of several highly non-trivial program transformations, such as Erosa and Hendren's goto-elimination procedure and the output of Ghidra decompiler. CF-GKAT opens up the application of Kleene Algebra to a wider set of challenges, and provides an important verification tool that can be applied to the field of decompilation and control-flow transformation.

==> sections/procedure.tex <==
% !TEX root=../paper.tex

\section{Decision procedure}%
\label{section:decision procedure}

To decide whether two CF-GKAT expressions denote the same guarded language, we propose CF-GKAT automata.
We will show that every CF-GKAT expression can be converted to a CF-GKAT automaton with the same continuation semantics, by induction on the expression \emph{à la Thompson~\cite{thompson_ProgrammingTechniquesRegular_1968}}.
However, because CF-GKAT automata implement the continuation semantics, directly comparing them for language equivalence will not be sufficient.
For instance, the following programs exhibit identical trace semantics, but differ in their continuation semantics:
\begin{mathpar}
  x := 1 \and \comAssert{\true}.
\end{mathpar}
The first program sets the indicator variable to 1, and the second program simply does nothing.
These programs have the same trace semantics, because the trace semantics does not care about the final value of the indicator variable.
Yet, their continuation semantics are different: guarded words in \(⟦x := 1⟧ᵢ^♯\) are always paired with the continuation \(\acc{1}\) regardless of \(i\), but \(⟦\comAssert{\true}⟧ᵢ^♯\) preserves the starting indicator by outputting the continuation \(\acc{i}\).
Furthermore, equivalence checking needs to account for jump resolution, by looking up the sequel of a trace ending in a continuation of the form $\jmp (i, \ell)$ in the traces starting from label $\ell$ with indicator value $i$.

Thus, our decision procedure does not rely equivalence checking of CF-GKAT automata; instead, we \emph{lower} the CF-GKAT automata into GKAT automata with the right semantics.
This allows us to reuse the nearly-linear decision procedure for GKAT automata equivalences~\cite{smolka_GuardedKleeneAlgebra_2020}.
Finally, the soundness and completeness of our decision procedure follows from the correctness of Thompson's construction (\Cref{the:thompson-correctness}), the correctness of the lowering (\Cref{the:cf-gkat-automaton-lowering-correctness}), and finally the correctness of GKAT automata equivalence checking~\cite{smolka_GuardedKleeneAlgebra_2020}.

\subsection{GKAT automata}

To establish our decision procedure, we will first recap GKAT automata and their trace semantics.
\begin{definition}[GKAT automata~\cite{smolka_GuardedKleeneAlgebra_2020, kozen_BohmJacopiniTheorem_2008a}]
 A \emph{GKAT automaton} $A ≜ ⟨ S, δ, \hat{s} ⟩$ consists of a set of \emph{states} $S$, a \emph{transition function} $\delta: S → \At → ⊥ + ⊤ + Σ × S$, and a \emph{start state} $\hat{s} ∈ S$.
\end{definition}
Intuitively, given a state $s$ and an atom $α$ accounting for the truth value of each primitive test, a GKAT automaton will either \emph{reject} the input, represented by $δ(s, α) = ⊥$; \emph{accept} the input, represented by $δ(s, α) = ⊤$; or to \emph{transition} to a new state in $S$ after executing an action from $Σ$, represented by $δ(s, α) ∈ Σ × S$.
A GKAT automaton induces a guarded language, by tracing all the possible execution paths reaching an accepting transition.

\begin{definition}
 Given a GKAT automaton $A ≜ ⟨ S, δ, \hat{s} ⟩$, we define $⟦ - ⟧_A: S → 𝒢$ as the (pointwise) smallest function satisfying the following rules for all $s ∈ S$ and $α ∈ \At$:
 \begin{mathpar}
  \inferrule{%
   δ(s, α) = ⊤
  }{%
   α ∈ ⟦ s ⟧_A
  }
  \and
  \inferrule{%
   δ(s, α) = (p, s') \\
   w ∈ ⟦ s' ⟧_A
  }{%
   αpw ∈ ⟦ s ⟧_A
  }
 \end{mathpar}
 Finally, we define the guarded language semantics of $A$ by setting $⟦ A ⟧ = ⟦ \hat{s} ⟧_A$.
\end{definition}

The trace equivalence of finite GKAT automata is decidable, which we record as follows.
\begin{theorem}[Decidability for GKAT~\cite{smolka_GuardedKleeneAlgebra_2020}]
 Given two finite GKAT automata $A₀$ and $A₁$, it is decidable whether they represent the same guarded language, i.e., whether $⟦ A₀ ⟧ = ⟦ A₁ ⟧$.
 The algorithm to do this has a complexity that is nearly-linear\footnote{$n ⋅ 𝒪(\hat{α}(n))$, where $\hat{α}$ is the inverse Ackermann function; c.f.~\cite{Tarjan75}.} in the total number of states.
\end{theorem}

\subsection{CF-GKAT automata}

To leverage the efficient decision algorithm for GKAT automata, we will need to convert each CF-GKAT expression $e$ and a starting indicator value \(i\) into a GKAT automaton that recognizes the guarded language $⟦ e ⟧\!↓ᵢ$.
As discussed, this process is separated into two steps, where we use CF-GKAT automata as an intermediate between CF-GKAT expressions and GKAT automata.
Like GKAT automata, CF-GKAT automata need a transition structure.
As it turns out having a separate type for this transition structure will turn out to be useful, so we isolate it as follows.
\begin{definition}[CF-GKAT dynamics]
 Given a set $S$, we write $G(S)$ for the set of possible \emph{CF-GKAT dynamics} on $S$, which is given by the following function type, where $C$ is as in \Cref{def:guarded-word-with-continuation}:
 \[G(S) ≜ I × \At → ⊥ + C + Σ × X × I.\]
 %FIXME: I think we need to fix the code to follow this type
\end{definition}

Intuitively, the elements of \(G(S)\) represent outgoing transitions of a single (initial) state or label in a CF-GKAT automaton over a state set $S$.
Given the current indicator value \(i ∈ I\) and an atom $α$ accounting for the truth value of each primitive test, a dynamics $ρ ∈ G(S)$ may either: \emph{reject} the input, represented by $ρ(i, α) = ⊥$; offer a \emph{continuation}, represented by $ρ(i, α) ∈ C$; or state in $S$, represented by $ρ(i, α) ∈ Σ × X × I$.

Then the definition of CF-GKAT automaton is similar to GKAT automaton, except we will need a function \(λ: L → G(S)\) where \(λ(ℓ)\) provides a dynamics representing the ``entry point'' of label \(ℓ\).
\begin{definition}
 A \emph{CF-GKAT automaton} \(A ≜ ⟨S, δ, \hat{s}, λ⟩\) consists of a set of \emph{states} \(S\), a \emph{transition function} \(δ: S → G(S)\),
 a \emph{start state} \(\hat{s} ∈ S\), and a \emph{jump map} \(λ: L → G(S)\).
\end{definition}

The transition map \(δ\) assigns every state a dynamics, while the jump map $λ$ assigns a dynamics to each label, indicating how to resume computation when a jump continuation is reached.

\begin{example}[A simple CF-GKAT automaton]%
\label{example:cf-gkat-automaton}
  Let $I = \{1,2\}$ and consider the following program:
  \[
    \comITE{t \wedge (x = 1)}{\{x := 2; \comLabel{ℓ};\; p\}}{\{x := 1;\; \comGoto{ℓ}\}}.
  \]
  We can construct the following automaton with the same continuation semantics from state $\hat{s}$:
  \[
    \begin{tikzpicture}
        \node (shat) {$\hat{s}$};
        \node[right=2cm of shat] (s) {$s$};
        \draw ($(shat) + (0mm, 7mm)$) edge[-latex] (shat);
        \draw (shat) edge[-latex] node[above] {\footnotesize $1,\{t\} \mid p, 2$} (s);
        \node[left=10mm of shat] (shatacc) {\footnotesize $\jmp (\ell, 1)$};
        \draw (shat) edge[double,double distance=2pt,-implies] node[above,align=center] {%
            \footnotesize $1, \emptyset$ \\[-1mm]
            \footnotesize $2, -$
        } (shatacc);
        \node[right=10mm of s] (sacc) {\footnotesize $\acc{i}$};
        \draw (s) edge[double,double distance=2pt,-implies] node[above] {\footnotesize $i, -$} (sacc);
    \end{tikzpicture}
  \]
  Here, \(ŝ \xrightarrow{1, \{t\} \mid p, 2} s\) means that \(δ(ŝ, 1, \{t\}) = (p, s, 2)\) and \(s \xRightarrow{i, -} \acc{i}\) means that \(δ(s, i, \alpha) = \acc{i}\) for $\alpha \in \At$ and $i \in I$.
  The behavior of this automaton, when starting from \(ŝ\), is as follows.
  \begin{itemize}
    \item
    If the input atom is \(\{t\}\) --- that is, the test $t$ is true --- and the indicator is $1$, we transition to the state \(s\), while setting the indicator to $2$ and executing \(p\) (and skipping over label $\ell$).
    Upon reaching $s$, the automaton accepts unconditionally, preserving the indicator.
    \item
    Otherwise, if the input atom is $\emptyset$ --- that is, the test $t$ is false --- or the indicator value is anything other than $1$, the automaton will simply offer the continuation \(\jmp{(ℓ,1)}\), thereby telling execution to continue from label $\ell$ with indicator value $1$.
  \end{itemize}
  As we can see, the behavior of \(ŝ\) indeed matches the behavior of the program when executing from the start.
  On the other hand, the entry dynamics for \(ℓ\) can be defined as follows:
  \[∀ i ∈ I, α ∈ \At, λ(ℓ, i, α) ≜ (p, s, i).\]
  To put the above definition into words: when jumping to the label \(ℓ\), we will reach the state \(s\) while executing \(p\).
  Thus, the behavior of \(λ(ℓ)\) matches the behavior of the program when starting from \(ℓ\).
\end{example}

\begin{remark}
We could have opted to instrument CF-GKAT automata with a \emph{state} for each label $\ell$, rather than a dynamics.
This would simplify their definition, at the cost of complicating the Thompson construction (\Cref{sec:thompson-construction}).
An additional advantage of this approach is that we avoid creating unreachable states when lowering CF-GKAT automata to GKAT automata (\Cref{sec:lowering-cf-gkat-automata-to-gkat}).
\end{remark}

To formalize the intuition of ``behaviors'', as seen in the previous example, we will assign a continuation semantics to each CF-GKAT automaton.
It is convenient to first assign a semantics to each dynamics \(ρ ∈ G(S)\) in a CF-GKAT automaton \(A ≜ ⟨S, δ, ŝ, λ⟩\), instead of every state.

\begin{definition}[continuation semantics]
 Given an automaton \(A ≜ ⟨S, δ, \hat{s}, λ⟩\),
 the continuation semantics of each dynamics \(ρ ∈ G(S)\) is an indexed family \(⟦ρ⟧_A: I → 𝒞\), defined as the (point-wise) smallest set satisfying the following rules for $i, j ∈ I$, $α ∈ \At$ and $c \in C$:
 \begin{mathpar}
  \inferrule{%
   ρ(i, α) = \acc{j}
  }{%
   α ⋅ \acc{j} ∈ (⟦ρ⟧_A)ᵢ
  }
  \and
  \inferrule{%
   ρ(i, α) = \brk{j}
  }{%
   α ⋅ \brk{j} ∈ (⟦ρ⟧_A)ᵢ
  }
  \and
  \inferrule{%
   ρ(i, α) = \ret
  }{%
   α ⋅ \ret ∈ (⟦ρ⟧_A)ᵢ
  }
  \\
  \inferrule{%
   ρ(i, α) = \jmp{(ℓ, j)}
  }{%
   α ⋅ \jmp{(ℓ, j)} ∈ (⟦ρ⟧_A)ᵢ
  }
  \and
  \inferrule{%
   ρ(i, α) = (p, s, j) \\
   w \cdot c ∈ (⟦δ(s)⟧_A)ⱼ
  }{%
   αpw \cdot c ∈ (⟦ρ⟧_A)ᵢ
  }
 \end{mathpar}
 Similar to the continuation semantics of expressions, the continuation semantics of automata are also labeled families of guarded languages with continuations: the semantics from the start \(⟦A⟧^♯\) is defined by the dynamics of the start state, and that of a label \(ℓ ∈ L\) is defined by the jump map:
 \begin{mathpar}
  ⟦ A ⟧^♯ = ⟦ δ(ŝ) ⟧_A, \and
  ⟦ A ⟧^ℓ = ⟦ λ(ℓ) ⟧_A \text{ for } ℓ ∈ L.
 \end{mathpar}
\end{definition}

\begin{example}
  Let the CF-GKAT automaton from \Cref{example:cf-gkat-automaton} be \(A\), we find that
\begin{mathpar}
  ⟦ A ⟧^♯_1 = \{ \emptyset \cdot \jmp{(\ell, 1)}, \{t\} p \emptyset \cdot \acc{2}, \{t\} p \{t\} \cdot \acc{2} \}
  \and
  ⟦ A ⟧^♯_2 = \{ \emptyset \cdot \jmp{(\ell, 1)}, \{t\} \cdot \jmp{(\ell, 1)} \}
  \and
  ⟦ A ⟧^ℓ_1 = ⟦ A ⟧^ℓ_2 = \{ \alpha p \beta \cdot \acc{i} : \alpha, \beta \in \At \}
\end{mathpar}
\end{example}

\subsection{Lowering CF-GKAT automata to GKAT automata}\label{sec:lowering-cf-gkat-automata-to-gkat}

The process to lower a CF-GKAT automaton $⟨S, δ, \hat{s}, λ⟩$ into a GKAT automaton consists of two different components.
We first ``embed'' the indicator values into the state set; the new state set then becomes $S × I$.
After that, we resolve all the continuations in transitions using the jump map.

The second step requires some care.
When $δ(s, i, α) = \jmp{(ℓ, j)}$, the $α$-transition leaving the state $(s, i)$ will take the behavior of \(ℓ\) starting from indicator \(j\) and atom \(α\), that is \(λ(ℓ, j, α)\).
This by itself is alright, but we also need to account for subprograms such as $\comLabel{l};\; x := k;\; \comGoto{\ell'}$, which entails that $λ(ℓ, j, α)$ points to a different label by returning $\jmp{(ℓ', k)}$.
%FIXME: many \jmp(ℓ, i) still have ℓ and i in the wrong place.
In turn, \(λ(ℓ', k, α)\) may also yield another jump, et cetera.
To resolve these chained jumps, we will need to iterate the jump map, and terminate when either the result is no longer a jump, or an infinite loop is detected.

\begin{definition}[iteration lifting]\label{def: iteration lifting}
  Given a function \(h: X → X + ⊥ + E\), where \(X\) is a finite set and \(⊥ + E\) specifies the ``exit results'', we can iterate $h$ until some exit value is reached, or a loop is detected.
  Formally, we define $\iter(h)$ as the least function satisfying for all $x \in X$ that
  \begin{mathpar}
    \iter(h)(x) =
        \begin{cases}
        \iter(h)(h(x)) & h(x) \in X \\
        h(x) & h(x) \in E
        \end{cases}
  \end{mathpar}
  in the directed-complete partial order (DCPO) on functions from $X$ to $X + \bot + E$ where $f \leq g$ when for all $x \in X$, we have that $f(x) = \bot$ or $f(x) = g(x)$.
  This makes $\iter(h)$ the least fixed point of the Scott-continuous function on this DCPO that sends $f$ to
  \[
    x \mapsto
        \begin{cases}
        f(h(x)) & h(x) \in X \\
        h(x) & h(x) \in E + \bot
        \end{cases}
  \]
  By Kleene's fixed point theorem this uniquely defines $\iter(h)$.
\end{definition}

\begin{remark}
  When $X$ is finite, we can directly compute $\iter(h)$ by iterating $h$.
  More precisely, we can define a helper function $\iter'(h): 2^X → X → ⊥ + E$ with an additional parameter, as follows:
  \begin{align*}
  \iter'(h) & (M)(x) ≜ \begin{cases}
      ⊥ & \text{if } x ∈ M  \\
      h(x) & \text{if } x ∉ M \text{ and } h(x) ∈ ⊥ + E \\
      \iter'(h)(M ∪ \{x\})(h(x)) & \text{if } x ∉ M \text{ and } h(x) ∈ X
    \end{cases};
  \end{align*}
  It is then not too hard to show that $\iter(h) = \iter'(h)(\emptyset)$.
  Intuitively, \(M\) keeps track of explored values in \(X\); if an input has already been explored, then \(\iter\) will return \(⊥\).
  On the other hand, if \(h(x)\) falls into the exit set \(⊥ + E\), then \(\iter(h)\) will exit and return \(h(x)\).
  Finally, if \(h(x)\) falls into \(X\), then \(\iter(h)\) will continue to iterate with \(h(x)\) as input, and mark \(x\) as explored.
  Note that \(\iter(h)\) is total because \(X\) is finite, so elements in \(X\) cannot be explored twice.
\end{remark}

For the sake of clarity, when defining a function \(h\) to iterate, we will write \(\contWith\) for the injection $X \to X + \bot + E$, so that $\contWith(x)$ indicates iteration continues with the value $x$; and $\exitWith$ for the injection \(⊥ + E → X + ⊥ + E\), so that $\exitWith(e)$ indicates iteration stops with the value $e$.

For jump resolution, iteration will continue when the result of \(λ\) is a jump, but exit otherwise.

\begin{definition}[Jump resolution]
 Let $S$ be a finite set, and let $λ: L → G(S)$ be a jump function.
 We define the resolved jump map ${λ\!↓}: L → G(S)$, as follows:
 \[
  {λ\!↓} = \iter \left(
    (ℓ, i, α) ↦ \begin{cases}
      \contWith (ℓ', i', α) & λ(ℓ, i, α) = \jmp{(ℓ', i')} \\
      \exitWith (λ(ℓ, i, α)) & \text{otherwise}
    \end{cases}
  \right)
 \]
\end{definition}

Because of the way $\iter$ works, this means that a cycle of $\jmp\!$-continuations (without actions in between) resolves to $\bot$.
Indeed, GKAT treats unproductive infinite iterations in the \command{while} loops with the same strategy~\cite{smolka_GuardedKleeneAlgebra_2020}, identifying non-terminating behavior with behavior that rejects explicitly.

Note that \(λ\!↓\) resolves all internal jumps, i.e., \(λ\!↓(\ell, i, \alpha)\) is never a jump continuation, because the iteration map used to define \(λ\!↓\) keeps iterating on values of this form.
We can then use the resolved jump map to tie together the loose ends indicated by jump continuations.
In the process, we can reroute continuations of the form $\brk i$ to rejection, as these should not occur at the top level of a well-formed program (internal $\brk\!$-continuations are handled in the next section).

\begin{definition}[Lowering]
 Given a CF-GKAT automaton \(A ≜ ⟨S, δ, \hat{s}, λ⟩\) and $i ∈ I$, we define the GKAT automaton \({𝐴\!↓ᵢ} ≜ ⟨S × I, δ\!↓, (\hat{s}, i)⟩\), where $δ\!↓$ is defined in two steps:
 \begin{align*}
  δ'((s, i), α) & ≜
    \begin{cases}
      λ\!↓(ℓ, i, α) & δ(s, i, α) = \jmp{(ℓ, i)} \\
      δ(s, i, α) & \text{otherwise}
    \end{cases}\\
  δ\!↓((s, i), α) & ≜
  \begin{cases}
    % \mathrlap and \hphantom is used for alignment purpose
    % the \mathrlap is the displayed expression
    % and \hphantom contains the "longest expression" for alignment
    \mathrlap{⊥}\hphantom{λ\!↓(ℓ, i, α)} & δ'(s, i, α) = \brk{j} \\
   ⊤ & \text{$δ'(s, i, α) = \ret$ or $\delta'(s, i, \alpha) = \acc{j}$} \\
   δ(s, i, α) & \text{otherwise}
  \end{cases}
 \end{align*}
\end{definition}
Note that $δ\!↓$ is well-defined: for all $s ∈ S$, $i ∈ I$ and $α ∈ \At$, it holds that $δ\!↓((s, i), α) ∈ ⊥ + ⊤ + Σ × (S × I)$, as expected for a GKAT automaton on state set $S × I$.

\begin{example}
If $A$ is the automaton from \Cref{example:cf-gkat-automaton}, then $\mathit{A}\! \downarrow _1$ is the following GKAT automaton:
\[
    \begin{tikzpicture}
        \node (shat1) {$(\hat{s}, 1)$};
        \node[right=of shat1] (s2) {$(s, 2)$};
        \node[left=of shat1] (s1) {$(s, 1)$};
        \draw ($(shat1) + (0mm, 7mm)$) edge[-latex] (shat1);
        \draw (shat1) edge[-latex] node[above] {\footnotesize $\{t\} \mid p$} (s2);
        \draw (shat1) edge[-latex] node[above] {\footnotesize $\emptyset \mid p$} (s1);
        \node[right=5mm of s2] (s2acc) {\footnotesize $\emptyset, \{t\}$};
        \draw (s2) edge[double,double distance=1.5pt,-implies] (s2acc);
        \node[left=5mm of s1] (s1acc) {\footnotesize $\emptyset, \{t\}$};
        \draw (s1) edge[double,double distance=1.5pt,-implies] (s1acc);
    \end{tikzpicture}
\]
Here, we use similar graphical conventions as before; for instance, $(\hat{s}, 1) \xrightarrow{\{ t \} \mid p} (s, 2)$ means that $\delta\!\downarrow((\hat{s}, 1), \{ t \}) = (p, (s, 2))$, and $(s, 2) \implies \emptyset, \{t\}$ means that $\delta\!\downarrow((s, 2), \emptyset) = \delta\!\downarrow((s, 2), \{t\}) = \top$.

In this lowered automaton, the jump continuation originally reached from $\hat{s}$ for indicator value $1$ and $t$ false (i.e., atom $\emptyset$) has been resolved via the jump map $\lambda$ to continue in state $s$.
This automaton also holds two copies of the state $s$, one for each possible indicator value; in this case, these states happen to have the same behavior, but in general they may be different.
\end{example}

Having defined our lowering operation, we can state its correctness as follows.

\begin{theorem}[Correctness of lowering]\label{the:cf-gkat-automaton-lowering-correctness}
 Let \(A ≜ ⟨S, δ, \hat{s}, λ⟩\) be a CF-GKAT automaton.
 The translation from CF-GKAT automata to GKAT automata commutes with the semantic jump resolution operator, in the sense that for $i ∈ I$, it holds that $⟦A\!↓_i⟧ = ⟦A⟧\!↓^♯ᵢ$.
\end{theorem}
\begin{proof}[Proof sketch]
More generally, we can prove that for any state $s$ of $A$, it holds that $⟦(s, i)⟧_{A\!↓_i} = G\!↓^♯ᵢ$, in which $G$ is the labeled family given by $G^\sharp = ⟦\delta(s)⟧_A$ and $G^\ell = ⟦\lambda(\ell)⟧_A$.
This property, which implies the main claim, can be proved by induction on the length of guarded words.
\end{proof}

\subsection{Converting expressions to CF-GKAT automata}\label{sec:thompson-construction}

The final piece of our puzzle is to convert CF-GKAT expressions to CF-GKAT automata.
To accomplish this, we generalize a construction proposed for GKAT, which turns a GKAT expression into a GKAT automaton in a trace-equivalent manner~\cite{smolka_GuardedKleeneAlgebra_2020}.
This construction, which was inspired by Thompson's construction to obtain a non-deterministic finite automaton from a regular expression~\cite{thompson_ProgrammingTechniquesRegular_1968}, proceeds by induction on the structure of the expression.
In contrast to the original, howvever, the Thompson construction for GKAT produces a GKAT automaton with a \emph{start dynamics}, also called an \emph{initial pseudostate}~\cite{smolka_GuardedKleeneAlgebra_2020}, instead of an explicit start state.
We adopt this shift in presentation to efficiently compose automata, avoiding the silent transitions in the original~\cite{thompson_ProgrammingTechniquesRegular_1968}.

\begin{definition}
 A CF-GKAT automaton with start dynamics \(A ≜ ⟨S, δ, ι, λ⟩\) consists of $S$, $δ$ and $λ$ as in a CF-GKAT automaton, in addition to a start dynamics \(ι ∈ G(S)\).
 The labeled family defined by a CF-GKAT automaton with start dynamics, also denoted $⟦A⟧$, is simply given by $⟦A⟧^\sharp = ⟦\iota⟧_A$ and $⟦ A ⟧^ℓ = ⟦ λ(ℓ) ⟧_A$, where the right-hand sides are defined as for plain CF-GKAT automata.
\end{definition}

It should be clear that CF-GKAT automata with start dynamics can easily be converted to plain CF-GKAT automata by adding a start state \(\hat{s}\) that takes the behavior of the start dynamics \(ι\):
\begin{equation}\label{cons: CF-GKAT pseudo start to CF-GKAT automata}
 ⟨S, δ, ι, λ⟩ ↦ ⟨S + \hat{s}, δ_ι, \hat{s}, λ⟩,
 \qquad
 \text{where}
 \qquad
 δ_ι(s, i, α) ≜
 \begin{cases}
  ι(i, α)    & \text{if } s = \hat{s} \\
  δ(s, i, α) & \text{if } s ≠ \hat{s}
 \end{cases}
\end{equation}

Our construction turns a CF-GKAT expression \(e\) into a CF-GKAT automaton with start dynamics, which we call the \emph{Thompson automaton for \(e\)}.
The following paragraphs describe the construction and intuition behind each case in the construction.
We make the simplifying assumption that each $\ell$ appears at most once in a subexpression of the form $\comLabel{\ell}$.
Moreover, we write \({!}\) for the unique function \({!}: ∅ → X\) (for any set $X$), and in inductive cases we denote the Thompson automata for \(e₁\) and \(e₂\) by \(A₁ ≜ ⟨S₁, δ₁, ι₁, λ₁⟩\) and \(A₂ ≜ ⟨S₂, δ₂, ι₂, λ₂⟩\) respectively.
Finally, to compress our notation, we will use the compact syntax of GKAT~\cite{smolka_GuardedKleeneAlgebra_2020} for \command{if}-statements and \command{while}-loops:
\begin{mathpar}
  e₁ +_b e₂ ≜ \comITE{b}{e₁}{e₂}, \and
  e₁^{(b)} ≜ \comWhile{b}{e₁}.
\end{mathpar}

\subsubsection*{Converting \command{break}, \command{return}, \command{goto}, and indicator assignment:}
recall that the semantics of \(\comBrk\), \(\comRet\), \(\comGoto{ℓ}\), and indicator assignments simply emit the corresponding continuations.
Thus, the non-trivial part of these Thompson automata are the start dynamics \(ι\), which output said continuations.
Because the start dynamics does not need to transition anywhere, there are no further states; because these programs also do not contain any $\comLabel\!$ primitives, there is no need to assign a dynamics for them either.
We thus construct the following automata:
\begin{align*}
  S_{\comBrk} & ≜ ∅ &
    δ_{\comBrk} & ≜ {!} &
    ι_{\comBrk}(i, α) & ≜ \brk{i} &
    λ_{\comBrk}(ℓ, i, \alpha) & ≜ ⊥ \\
  S_{\comRet} & ≜ ∅ &
    δ_{\comRet} & ≜ {!} &
    ι_{\comRet}(i, α) & ≜ \ret &
    λ_{\comRet}(ℓ, i, \alpha) & ≜ ⊥ \\
  S_{\comGoto{ℓ}} & ≜ ∅ &
    δ_{\comGoto{ℓ}} & ≜ {!} &
    ι_{\comGoto{ℓ}}(i, α) & ≜ \jmp{(ℓ, i)} &
    λ_{\comGoto{ℓ}}(ℓ, i, \alpha) & ≜ ⊥ \\
  S_{x := i} & ≜ ∅ &
    δ_{x := i} & ≜ {!} &
    ι_{x := i}(i, α) & ≜ \acc{i} &
    λ_{x := i}(ℓ, i, \alpha) & ≜ ⊥
\end{align*}

\subsubsection*{Converting tests and primitive actions:}
the conversions of primitive tests and primitive actions largely inherit the Thompson construction for GKAT\@.
The Thompson automaton for tests \(\comAssert{b}\) contains only a start dynamics, which accepts the input indicator-atom pairs if and only if they satisfy \(b\).
The Thompson's automata for primitive actions \(p\) contains a start dynamics that always executing the action \(p\) before transitioning to the unique state, which accepts unconditionally.
\begin{align*}
  S_{\comAssert{b}} & ≜ ∅ &
    S_{p} & ≜ \{*\} \\
  δ_{\comAssert{b}} & ≜ {!} &
    δ_{p}(s, i, α) & ≜ \acc{i} \\
  ι_{\comAssert{b}}(i, α) & ≜ \begin{cases}
      \acc{i} & (i, α) ∈ ⟦b⟧ \\
      ⊥ & (i, α) ∉ ⟦b⟧
    \end{cases} &
    ι_{p}(i, α) & ≜ (p, *, i) \\
  λ_{\comAssert{b}}(ℓ, i, \alpha) & ≜ ⊥ &
    λ_{p}(ℓ, i, \alpha) & ≜ ⊥
\end{align*}

\subsubsection*{Converting labels:}
recall that \(\comLabel{ℓ'}\) is a does not affect the semantics from the start of the program, i.e., should be the same as the sequential identity \(\comAssert{\true}\).
However, the behavior of \(\comLabel{ℓ'}\) and \(\comAssert{\true}\) diverges when we consider the jump map: if $\ell = \ell'$, then executing $\comLabel{\ell'}$ starting from $\ell$ lets us reach the end of the program, whereas $\comAssert{\true}$ does not contain any label.
We thus end up with the following Thompson automaton for $\comLabel{\ell'}$:
\begin{align*}
  S_{\comLabel{ℓ'}} & ≜ ∅ &
  δ_{\comLabel{ℓ'}} & ≜ {!} &
  ι_{\comLabel{ℓ'}}(i, α) & ≜ \acc{i} &
  λ_{\comLabel{ℓ'}}(ℓ, i, α) & ≜ \begin{cases}
    \acc{i} & ℓ = ℓ'  \\
    ⊥ & ℓ ≠ ℓ'
  \end{cases}
\end{align*}

% FIXME: I think this is too on the nose... Basically just reiterating the definition
% TK: I think it's unavoidable at this point
\subsubsection*{Converting \command{if} statements:}
the Thompson automaton for \(\comITE{b}{e₁}{e₂}\) is also similar to that of GKAT\@: if the input indicator-atom pair satisfies (resp.\ falsifies) \(b\), the start \(ι\) will enter the Thompson automaton of \(e₁\) (resp.\ $e_2$) by taking on the behavior of \(ι₁\) (resp.\ $\iota_2$).
The jump map \(λ\) assigns the entry point for label \(ℓ\) based on where \(ℓ\) appears: namely if \(ℓ\) appears in \(e₁\), then \(ℓ\) will take its entry point in \(A₁\); and similarly, if \(ℓ\) appears in \(e₂\), \(ℓ\) will take its entry point in \(A₂\).
\begin{minipage}{0.54\textwidth}
  \begin{align*}
  S_{e₁ +_b e₂} & ≜ S₁ + S₂ \\
  λ_{e₁ +_b e₂}(ℓ) & ≜ \begin{cases}
    λ₁(ℓ) & (\comLabel{ℓ}) \text{ appears in } e₁\\
    λ₂(ℓ) & (\comLabel{ℓ}) \text{ appears in } e₂\\
    ⊥ & \text{otherwise}
  \end{cases}
  \end{align*}
\end{minipage}
\begin{minipage}{0.44\textwidth}
\begin{align*}
  δ_{e₁ +_b e₂}(s) & ≜ \begin{cases}
    δ₁(s) & \text{if } s ∈ S₁ \\
    δ₂(s) & \text{if } s ∈ S₂ \\
  \end{cases} \\
  ι_{e₁ +_b e₂}(i, α) & ≜ \begin{cases}
    ι₁(i, α) & (i, α) ∈ ⟦b⟧ \\
    ι₂(i, α) & (i, α) ∉ ⟦b⟧
  \end{cases}
\end{align*}
\end{minipage}

\subsubsection*{Converting Sequencing:}
Sequencing of automata can be defined by \emph{uniform continuations}~\cite{smolka_GuardedKleeneAlgebra_2020}, which combine two dynamics $h₁, h₂ ∈ G(S)$ into a new dynamics \(h₁[h₂]\).
The latter acts like $h₁$ in almost all cases, except when $h₁$ accepts --- then it will take on the behavior of \(h₂\).
In other words, \(h₁[h₂]\) connects all the accepting transition of \(h₁\) to \(h₂\).
Uniform continuation is typically used to compose two automata or add self-loops to an automaton; it can be formally defined as follows.
\begin{definition}[Uniform Continuation]
  Let $S$ be a set and given two dynamic $h₁, h₂ ∈ G(S)$,
  their \emph{uniform continuation} is the dynamic $h₁[h₂] ∈ G(S)$, defined as follows:
  \[
    h₁[h₂](i, α) ≜
    \begin{cases}
    h₂(i', α) & \text{if } h₁(i, α) = \acc{i'} \\
    h₁(i, α)  & \text{otherwise}
    \end{cases}
  \]
\end{definition}
To construct the Thompson automaton for \(e₁; e₂\), we will simply connect all the accepting transitions in \(A₁\) to \(A₂\) by applying uniform continuations on start dynamics \(ι₁\), transitions \(δ₁\), and jump map \(λ₁\), while preserving the dynamics in \(A₂\) --- with the proviso that, if $\ell$ accepts in $A_1$, then computation continues in $A_2$ via a uniform extension with $\iota_2$.
Formally, this works out as follows:
\begingroup%
\allowdisplaybreaks%
\begin{align*}
  S_{e₁; e₂} & ≜ S₁ + S₂ &
  ι_{e₁; e₂} & ≜ ι₁[ι₂] \\
  δ_{e₁; e₂}(s) & ≜ \begin{cases}
    δ₁(s)[ι₂] & \text{if } s ∈ S₁ \\
    δ₂(s) & \text{if } s ∈ S₂ \\
  \end{cases} &
  λ_{e₁; e₂}(ℓ, i, α) & ≜ \begin{cases}
    λ₁(ℓ)[\iota_2] & (\comLabel{ℓ}) \text{ appears in } e₁\\
    λ₂(ℓ) & (\comLabel{ℓ}) \text{ appears in } e₂\\
    ⊥ & \text{otherwise}
  \end{cases}
\end{align*}
\endgroup%

\subsubsection*{Converting \command{while} loops:}
Like GKAT automata, CF-GKAT automata require every transition between states to execute a primitive action.
This presents a unique challenge in defining the start dynamics for while loops.
Namely, a loop may not immediately encounter a primitive action on its first iteration, but this may trigger a change in indicator value that causes a primitive action to be executed in the \emph{next} iteration, or the one after that, et cetera.
This is reminiscent of jump resolution, where we also have to chase through some indirection to arrive at the right transition.

As a concrete example of this phenomenon, consider the following CF-GKAT program:
\begin{equation}%
\label[prog]{prog:loop-head-iter-example}
  \begin{aligned}
    \comWhile{\true}{\{
      & \comITE{x = 0}{x := 1 \\
      &}{\comITE{x = 1}{\comBrk
      }{\{\; \comAssert{\true} \;\}}} \;\}}
  \end{aligned}
 \end{equation}
 If this program starts with the indicator $0$, then the first continuation (\(\brk{1}\)) will be encountered on the second iteration of the loop.
Even worse, when starting with an indicator value like \(x = 2\), the program will enter an infinite loop and never encounter a primitive action or continuation.

Fortunately, these difficulties can be resolved by the \(\iter\) function (\Cref{def: iteration lifting}): we repeat the start of the loop body until we encounter some productive behavior, or we get stuck.
\begin{definition}[Iterated Start Dynamics]
  Let $S$ be a set, let $h ∈ G(S)$, and $b ∈ \BExp$.
  We can use the \(\iter\) function to define $hᵇ: G(S)$, as follows:
  \[
   h^b ≜
   \iter\left(
     (i, α) ↦
     \begin{cases}
       \exitWith(\acc{i}) & \text{if } (i, α) ∉ ⟦b⟧ \\
       \contWith(i', α) & \text{if } (i, α) ∈ ⟦b⟧ \text{ and } h(i, α) = \acc{i'} \\
       \exitWith(h(i, α)) & \text{otherwise}
     \end{cases}
   \right)
  \]
\end{definition}
In the first case, the input \((i, a)\) doesn't satisfy \(b\), causing the while loop to terminate.
In the second case, the loop body accepts \((i, α)\) immediately and returns the exit indicator value \(i'\), thus the iteration of loop body will continue with \((i', α)\).
And the final case is reached when the program executes an action or encounters a non-local control, then the iteration can also be stopped.
\begin{example}[Iterated Start Dynamics]
  Consider~\cref{prog:loop-head-iter-example} above with indicator set \(\{0, 1, 2\}\), no primitive action, no label, and no primitive test.
  Then the only atom is \(∅\), and Thompson's automaton \(A₁ ≜ ⟨S₁, δ₁, ι₁, λ₁⟩\) for the loop body can be computed to be as follows:
  \begin{align*}
    && ι₁(0, ∅) & ≜ \acc{1} &&&\\
    S₁ & ≜ ∅ &
    ι₁(1, ∅) & ≜ \brk{1} &
    δ₁ & ≜ {!} &
    λ(\ell, i, \alpha) & ≜ \bot \\
    && ι₁(2, ∅) & ≜ \acc{2} &&&
  \end{align*}
  Then we compute the iterated start dynamics \(ι^{\true}\) with input \((0,∅)\) and \((2,∅)\):
  \begin{align*}
    {ι₁}^{\true}(0, ∅)
    & = {ι₁}^{\true}(1, ∅)
      & \text{because }(0, ∅) ∈ ⟦\true⟧ \text{ and } {ι₁}(0, ∅) = \acc{1} \\
    & = \brk{1}
      & \text{because } {ι₁}(1, ∅) = \brk{1} \\[5px]
    {ι₁}^{\true}(2, ∅)
    & = {ι₁}^{\true}(2, ∅)
      & \text{because }(2, ∅) ∈ ⟦\true⟧ \text{ and } ι₁(2, ∅) = \acc{2} \\
    & = ⊥
      & \text{because the input \((2, ∅)\) is already explored}
  \end{align*}
\end{example}

With the start dynamics defined, we still need to resolve structures within the loop body, like the \(\comBrk\)-continuation.
To perform $\comBrk$-resolution, we extend the \(⌊-⌋\) operator to dynamics.
\begin{definition}
Let $S$ be a set, and let $h ∈ G(S)$.
We define $⌊h⌋ ∈ G(S)$ by lifting \(h\) via \(⌊-⌋\) (c.f. \Cref{def:intermediate-sequencing-loops}) when it returns a continuation, that is to say:
\[
  ⌊h⌋(i, α) = \begin{cases}
  ⌊h(i, α)⌋ & \text{if } h(i, α) ∈ C \\
  h(i, α)   & \text{otherwise}
  \end{cases}
\]
\end{definition}

Finally, the transition function \(δ\) and jump map \(λ\) can be defined by first connecting \(δ₁\) and \(λ₁\) back to start dynamics \(ι\), forming a loop in the automaton;
then resolving the \(\brk{i}\) continuations using \(⌊-⌋\).
Formally, the Thompson automaton for loop \(e^{(b)}\) can then be defined as follows:
\begin{align*}
  S_{e₁^{(b)}} & ≜ S₁ &
  δ_{e₁^{(b)}} & ≜ ⌊ δ₁(s)[{ι₁}^{b}] ⌋ &
  ι_{e₁^{(b)}} & ≜ ⌊ {ι₁}^{b} ⌋ &
  λ_{e₁^{(b)}}(ℓ) & ≜ ⌊ λ(ℓ)[{ι₁}^{b}] ⌋
\end{align*}
Note how in the case of the jump map, we resolve $\brk\!$-continuations after the uniform continuation with the iterated start dynamics.
This way, a jump to a label inside the loop that hits a $\comBrk$ statement immediately will continue executing execution after the loop, as is to be expected.

% FIXME: I think this is good to say, but should be in a separate remark after the construction is fully presented - T
% In the worst case, it is possible for \(I'\)
% to exhaust all of \(I\) before an infinite loop is found,
% which means computing \(γ\) can take \(|I|\) time
% for every indicate \(i\) and atoms \(α\).
% However, for a fixed atom \(α\), we can cache the result of each \(i\),
% leading to a \(|I|\)-timed algorithm to compute \(γ\) for every input \(i\).

The correctness of the Thompson construction for CF-GKAT can be formulated as follows:
\begin{theorem}[Thompson's construction preserves the continuation semantics]\label{the:thompson-correctness}
  Given an expression $e ∈ \Exp$, let $A_e$ be the Thompson automaton for $e$, then \(⟦e⟧ = ⟦A_e⟧\).
  More specifically, by unfolding the definition of continuation semantics, this boils down to the following:
  \[∀ i ∈ I, ℓ ∈ ♯ + L, ⟦e⟧ᵢ^ℓ = ⟦A_e⟧ᵢ^ℓ\]
 \end{theorem}
 \begin{proof}[Proof sketch]
 By induction on $e$.
 This proof is somewhat tedious, but ultimately doable.
 The inductive cases are very similar to the ones for the Thompson construction in plain GKAT~\cite{smolka_GuardedKleeneAlgebra_2020}; the only difference is that, this time, the semantics of the jump map needs to be taken into account.
 \end{proof}

\subsection{Algorithm, Completeness, and Complexity}

With the definitions of lowering and Thompson's construction established, the decision procedure mostly follows.
Nevertheless, it remains essential to define the alphabets $\Sigma$, $T$, $I$, and $L$, representing the set of primitive actions, primitive tests, indicator values, and labels, respectively.
We may safely restrict primitive actions, primitive tests, and labels to those explicitly present in the expression, as expanding the alphabet beyond these will preserve (the equational theory of) the trace semantics.
This trace is a property that can be validated by induction on the expression itself.

The set of indicator values, however, occupies a unique position.
If the initial indicator value is absent from the program, the program's traces may diverge from traces starting from the present indicator values.
\Cref{prog:loop-head-iter-example} is one of the witnesses of this phenomenon: if the initial indicator value is 0 or 1, the program terminates; however, when starting from an indicator value that doesn't appear in the program, the program will loop indefinitely.
An even simpler example is
\(\comAssert (x = 1); p,\)
which executes \(p\) if the initial indicator value is 1, but rejects when started with indicator values that are not present in the program.
Fortunately, given an expression \(e\), it is not hard to show that if neither \(i\) nor \(i'\) appears in \(e\), then the behaviors for both values coincide, i.e.,
\(∀ ℓ, ⟦e⟧_{i'}^{ℓ} = ⟦e⟧ᵢ^{ℓ}.\)
Thus, when gathering the indicator values, it suffices to take those that appear explicitly in the program augmented with a fresh value \(*\) that does not appear in the program.


We summarize our decision procedure as follows:
\begin{enumerate}
  \item
  Given two CF-GKAT programs \(e, f\), we first collect their alphabets $\Sigma$, $T$, $I$, and $L$.
  We gather the sets of primitive actions \(\Sigma\), primitive tests \(T\), and labels \(L\) that are present in either \(e\) or \(f\).
  Additionally, we identify the set of indicator values \(I\), encompassing those found in either \(e\) or \(f\), along with an additional indicator \(*\) that is exclusive to both programs.
  \item
  We then proceed to compute the Thompson automata of \(e\) and \(f\) and convert them into CF-GKAT automata, denoted as \(A_e\) and \(A_f\).
  It is noteworthy that these automata preserve the continuation semantics (\Cref{the:thompson-correctness}).
  Formally,
  \begin{mathpar}
    ⟦A_e⟧ = ⟦e⟧ \and ⟦A_f⟧ = ⟦f⟧.
  \end{mathpar}
  \item
  Subsequently, we lower both \(A_e\) and \(A_f\) to GKAT automata \(A_e\!↓ᵢ\) and \(A_f\!↓ᵢ\) for each \(i ∈ I\).
  By \Cref{the:cf-gkat-automaton-lowering-correctness}, the latter exhibits the same traces as \(e\) and \(f\) starting from \(i\):
  \begin{mathpar}
    ⟦A_e \!↓ᵢ⟧ = ⟦A_e⟧\!↓ᵢ = ⟦e⟧\!↓ᵢ, \and
    ⟦A_f \!↓ᵢ⟧ = ⟦A_f⟧\!↓ᵢ = ⟦f⟧\!↓ᵢ.
  \end{mathpar}
  \item
  Finally, we run the equivalence algorithm for GKAT automata~\cite{smolka_GuardedKleeneAlgebra_2020} on \(A_e \!↓ᵢ\) and \(A_f \!↓ᵢ\) for each \(i ∈ I\), and return true when all the GKAT automata equivalence checks return true.
\end{enumerate}

\paragraph*{Soundness and completeness:}
The soundness and completeness of this algorithm now follow as a corollary of the corresponding properties for the decision procedure in GKAT\@.
We denote the algorithm introduced above as \(\mathrm{equiv}_{\mathsf{CFGKAT}}\), while the decision algorithm for equivalence of GKAT automata is denoted as \(\mathrm{equiv}_{\mathsf{GKAT}}\).
Thus, we establish the equivalence:
\begin{align*}
  \mathrm{equiv}_{\mathsf{CFGKAT}}(e, f)
  & ⟺ ∀ i ∈ I, \mathrm{equiv}_{\mathsf{GKAT}}(A_e \!↓ᵢ, A_f \!↓ᵢ)  \\
  & ⟺ ∀ i ∈ I, ⟦A_e \!↓ᵢ⟧ = ⟦A_f \!↓ᵢ⟧ \\
  & ⟺ ∀ i ∈ I, ⟦e⟧\!↓ᵢ = ⟦f⟧\!↓ᵢ \\
  & ⟺ ⟦e⟧\!↓ = ⟦f⟧\!↓.
\end{align*}
Thus, \(e\) and \(f\) are trace equivalent if and only if \(\mathrm{equiv}_{\mathsf{GKAT}}(e, f)\) returns true.

\paragraph*{Algorithm complexity:}
We now give a rough account of the computational cost for deciding equivalence of CF-GKAT programs.
Like GKAT, we consider $T$ to be fixed for the purpose of analyzing complexity; otherwise, deciding equivalence of (CF-)GKAT programs is co-NP hard~\cite{smolka_GuardedKleeneAlgebra_2020}.

Starting with an expression \(e\), we observe that the number of states in the Thompson automaton \(A_e\) is bounded by \(|e|\), which is the size of $e$ as a term.
While computing this automaton we must bear in mind that deriving the iterated start dynamics of a loop using $\iter$ may take up to $|I|$ steps (assuming we use memoization to compute the output for each input), and this happens at most $|e|$ times.
After lowering, each GKAT automaton \(A_e\!↓\) contains at most \(|I|×|e|\) states, and computing the jump resolution using $\iter$ takes on the order of $|L| \times |I|$ steps (again using memoization).

For each \(i ∈ I\), determining the equivalence between \(A_e\!↓ᵢ\) and \(A_f\!↓ᵢ\) is accomplished in (nearly\footnote{We omit the factor coming from the inverse Ackermann function $\hat{\alpha}(n)$, which is at most $5$ for any realistic number of states, out of consideration for the sake of simplicity.}) linear time relative to the number of states, so this check takes about \(|I|×(|e|+|f|)\) steps.
To verify trace equivalence between \(e\) and \(f\), this check is required for \(A_e\!↓ᵢ\) and \(A_f\!↓ᵢ\) across all \(i∈I\).

Therefore, the overall time spent on the equivalence checks is on the order of \(|I|^2 × (|e|+|f|)\), while computing the automata can take roughly $|L| \times |I| + |I| \times (|e| + |f|)$ time.
This implies that the algorithm's complexity scales (nearly) linearly with the sizes of \(e\) and \(f\), linearly in the size of $L$, and quadratically with respect to the number of indicator values \(|I|\).


==> sections/related_work.tex <==
% !TEX root=../paper.tex

\section{Related Work}%
\label{sec:related-work}

% We identify and discuss related work in three distinct areas.
% Kleene algebra, program equivalence, and abstract interpretation.

\subsection{(De)compiler Verification and Validation} % chktex 36

Because we anticipate that the primary use case of CF-GKAT is the verification and validation of (de)compilers, we briefly go over existing work in this area, and relate it to ours. % chktex 36

\smallskip
\emph{Compiler verification and validation} is a well-developed research area.
The most rigorous approach is to use a proof assistant to verify the compilation algorithm relative to a formal semantics of the source and target language~\cite{leroy_CompCertFormallyVerified_2016,tan-etal-2016,neis-etal-2015}.
This method offers a foundational guarantee of correctness without imposing runtime overhead, but can be challenging and time-consuming to adapt on a large scale.
We envision that CF-GKAT could be used to automate correctness proofs of program transformations (provided that CF-GKAT equivalence is sound w.r.t.\ the language semantics).

Compiler testing feeds synthesized programs into different or differently configured compilers, and compares the resulting programs~\cite{chen_SurveyCompilerTesting_2021a,le_CompilerValidationEquivalence_2014a,yang_FindingUnderstandingBugs_2011}.
While this approach does not provide any formal guarantee of correctness, it has been effective in finding compiler bugs~\cite{yang_FindingUnderstandingBugs_2011}.
Within this framework, CF-GKAT could be used as an equivalence checking oracle; however, because our work is limited to \emph{control-flow} equivalence, a blinding pass (similar to our experiments above) is likely necessary.

Translation validation~\cite{goldberg_LoopsPracticalIssues_2005,kasampalis_LanguageparametricCompilerValidation_2021,necula_TranslationValidationOptimizing_2000,kasampalis_TranslationValidationCompilation_2021,zhang_FormalVerificationOptimizing_2018,pnueli-etal-1998,sewell-etal-2013} scales well \emph{and} offers formal guarantees.
This is achieved through the use of symbolic evaluations and bisimulation to generate verification conditions for SMT solvers, allowing the validator to handle both data-flow and control-flow transformations simultaneously, albeit at the cost of decidability. Some approaches also employ graph isomorphism checks~\cite{awadhutkar-etal-2022}, which can be more computationally expensive than bisimulation.
Compared to other efforts, our focus is exclusively on control-flow transformations.
This allows us to work with a minimal language, sufficient to cover well-known control-flow transformations~\cite{yakdan_NoMoreGotos_2015,erosa-hendren-1994,DBLP:journals/cacm/BohmJ66,grathwohl_KAT_2014}, and establish meta-properties such as correctness of our decision procedure and low complexity --- all of which are properties out of reach for unabstracted (Turing-complete) languages.

Predicate abstraction~\cite{ball-etal-2001} can help focus on relevant parts of a program prior to analysis, which makes it similar to blinding.
However, predicate abstraction requires input on \emph{how} to abstract the program, whereas blinding abstracts away all parts that are not relevant to flow control.

\smallskip
\emph{Decompiler verification and validation} is, by comparison, not as explored as compiler verifcation and validation.
Again, a distinction can be made between verification~\cite{DBLP:conf/pldi/VerbeekBFR22}, validation~\cite{dasgupta_ScalableValidationBinary_2020} and testing~\cite{liu-wang-2020,cao-etal-2024}.
Current efforts in verification and validation focus on \emph{lifting}, i.e., decoding machine code into assembly instructions or some other intermediate representation~\cite{ccs24verbeek,DBLP:conf/pldi/VerbeekBFR22,dasgupta_ScalableValidationBinary_2020}.
There has been some preliminary work on developing a sound decompiler that can produce C code, control-flow structuring is limited~\cite{DBLP:conf/sefm/VerbeekOR20}.
This constitutes a prime use case for CF-GKAT\@.

\subsection{Kleene Algebra And Control-Flow Verification}

Existing work has explored non-local control-flow structures and indicator variables within the framework of KAT, albeit with a number of differences from our work.  

Kozen characterized the semantics for programs with non-local control-flow structures as a family of KAT expressions~\cite{kozen_NonlocalFlowControl_2008a}.
This approach yields a decision procedure for program equivalences, by reducing them to KAT equivalences.
In contrast, CF-GKAT takes a more explicit approach by defining the continuation semantics, and the equivalence is computed by converting programs directly into automata.
Our method closed an open question by \citet{kozen_NonlocalFlowControl_2008a}, on whether non-local control-flow structures can be treated ``directly'', without being converted into KAT expressions.

\citet{grathwohl_KAT_2014} proposed \emph{KAT+B!} an extension of KAT with ``mutable tests'', which can be thought of as indicator variables with \(I = \{\true, \false\}\).
Concretely, their setter \(b!\) equates to indicator assignment \(x = \true\) and \(\overline{b}!\) to \(x = \false\); similarly, their tester \(b?\) corresponds to primitive indicator tests. % chktex 40
Although this is a special case of indicator variable, KAT+B!\@ can simulate indicator variable over a finite set \(I\) with \(|I|\) mutable tests.
% For example, indicator assignments $x := i$ can be simulated by ${b_i!} ; Π_{i' ≠ i}(\overline{b_{i'}}!)$, where each mutable test \(b_i\) records whether the indicator variable \(x\) is assigned to \(i\). 
We opt to treat indicator assignments and tests as primitives, rather than restricting ourselves to (boolean-valued) mutable tests.

Our treatment of indicator variables also draw inspirations from NetKAT~\cite{anderson_NetKATSemanticFoundations_2014a}. 
Specifically, NetKAT can be seen as a special case of KAT with indicator variables, the only primitive action is \texttt{dup}.
KATch~\cite{moeller-etal-2024}, a fast symbolic equivalence checker for NetKAT, is of particular interest to us in this space.
In the future, we hope to scale our equivalence checker using similar symbolic techniques.

To reason about variable assignment beyond indicator variables, Schematic KAT~\cite{angus_KleeneAlgebraTests_2001} provides a fine-grained algebraic theory for assignments over uninterpreted functions.
Later, Schematic KAT was also extended to reason about local variables~\cite{aboul-hosn_LocalVariableScoping_2008a}.
Neither work covers the complexity of the equivalence problem for schematic KAT and its extensions.
Kleene algebra can also be extended with nominal techniques~\cite{kozen_CompletenessIncompletenessNominal_2015,kozen_NominalKleeneCoalgebra_2015,gabbay_FreshnessNameRestrictionSets_2011}, which may help to reason about potentially infinite data domains, although the inclusion of tests to nominal Kleene algebra has not yet been investigated.

Separately, \citet{kozen_CertificationCompilerOptimizations_2000b} have applied KAT to verify compiler correctness. 
Their system directly uses postulated equalities for parts of their verification task. 
In contrast, our framework is based on the trace semantics, a commonly accepted semantics for \command{while}-programs.

\subsection{Complexity And Expressivity}

Finally, unlike the systems above, our system is based on GKAT, instead of KAT\@. 
This enhances the scalability of our equivalence checking algorithms to accommodate larger programs: whereas equivalence of KAT expressions is PSPACE-complete~\cite{cohen-kozen-smith-1996}, equivalence of CF-GKAT expressions can be verified in polynomial time for a fixed number of tests~\cite{smolka_GuardedKleeneAlgebra_2020}.
Symbolic techniques previously applied to KAT may also provide better ways of mitigating the complexity of tests~\cite{pous-2015}.

Our system is the first to integrate both indicator variables and non-local control flow in a unified framework, which enables the verification of complex control-flow transformations that leverage both indicator variables and non-local control flow~\cite{yakdan_NoMoreGotos_2015}.
Our notion of trace equivalence is also coarser than previous systems; CF-GKAT equates programs ending in different indicator values:
\[
    \begin{array}{c}
    x := \true; \comITE{x = \true}{\command{print(1)}}{\command{print(2)}} \\[1mm]
    x := \false; \comITE{x = \false}{\command{print(1)}}{\command{print(2)}}
    \end{array}
\]
The two programs above are equivalent to an outside observer, as both of them will print 1; yet the assignment of \(x\) is different at the end of the program, thus systems like KAT+B!~\cite{grathwohl_KAT_2014} will not equate these two programs.
On the other hand, our equivalence is not a congruence.
For example,  $(x := 1) ≡ (x := 0)$ holds in CF-GKAT, because we disregard the different ending indicator values \(1\) and \(0\), while $(x := 1); \comAssert{(x = 1)}$ is not equivalent to $(x := 0); \comAssert{(x = 1)}$, even in CF-GKAT --- the former program always succeeds, while the latter always fails.

% \subsection{Program equivalence} %or program reasoning? or do we need this at all?

% Showing that two programs are equivalent is a fundamental problem that has been approached from many different angles.
% Several works stand out, when we consider showing equivalence of two programs, in the context of program transformation.
% In compilation, the most prominent work is that of Leroy~\cite{DBLP:journals/cacm/Leroy09}, where he introduces a formally verified C compiler.
% Each transformation step of the compiler has been proven to be semantically equivalent.

% \subsection{Abstract interpretation}

% The approach presented in this paper can be regarded as a form of abstract interpretation\cite{DBLP:conf/popl/CousotC77,DBLP:conf/popl/CousotC79}.
% In abstract interpretation, static analysis is performed by approximating the semantics of a program by mapping concrete program states to an abstract domain.
% One could argue that the approach presented in this paper fits that description.
% In the context of this publication, several abstract interpretation approaches are relevant.

% Value Set Analysis (VSA) is an instance of abstract interpretation.
% VSA is used to determine which values a variable or expression can take.


% % some works on value set analysis:

% % JAKSTAB uses abstract interpretation to resolve indirections in decompilation
% \cite{DBLP:conf/cav/KinderV08,DBLP:conf/vmcai/KinderZV09}
% % CodeSurfer/x86 analyzes x86 binaries using VSA
% \cite{DBLP:conf/cc/BalakrishnanGRT05}
% % BAP also does this
% \cite{DBLP:conf/cav/BrumleyJAS11}


% %uses abstract interpretation to recover information about binaries, including memory accesses (which is the abstract part).
% \cite{DBLP:conf/cc/BalakrishnanR04}
% \cite{DBLP:conf/cc/RepsB08}


